Unsupervised Distillation of Syntactic Information from Contextualized Word Representations

Contextualized word representations, such as ELMo and BERT, were shown to perform well on various semantic and syntactic tasks. In this work, we tackle the task of unsupervised disentanglement between semantics and structure in neural language representations: we aim to learn a transformation of the contextualized vectors, that discards the lexical semantics, but keeps the structural information. To this end, we automatically generate groups of sentences which are structurally similar but semantically different, and use metric-learning approach to learn a transformation that emphasizes the structural component that is encoded in the vectors. We demonstrate that our transformation clusters vectors in space by structural properties, rather than by lexical semantics. Finally, we demonstrate the utility of our distilled representations by showing that they outperform the original contextualized representations in a few-shot parsing setting.

==> equivalent_sentences.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{lllll}
% \multicolumn{5}{l}{{\color{red} Despite} its {\color{blue} comparatively} large {\color{orange}{geographic}} size , the population of washington county was {\color{cyan}{sparse}} and small .}             \\
% \multicolumn{5}{l}{{\color{red} Despite} its {\color{blue}{nearly}} contiguous {\color{orange}{modern}} position , the soil of morris sford was {\color{cyan}{distant}} and lifeless .}                      \\
% \multicolumn{5}{l}{{\color{red} Despite} its {\color{blue}{particularly}} strategic {\color{orange}{high}} terrain , the density of jasper territory was {\color{cyan}{shallow}} and broad .}                \\
% \multicolumn{5}{l}{{\color{red} Despite} its {\color{blue}{significantly}} major {\color{orange}{topographic}} history , the collection of newport cemeteries was {\color{cyan}{expensive}} and necessary .} \\
% \multicolumn{5}{l}{{\color{red} Despite} its {\color{blue}{increasingly}} prominent {\color{orange}{current}} use , the music of clarke shakespeare was {\color{cyan}{dense}} and strong}


\multicolumn{5}{l}{{\color{red} After} completing his {\color{blue} national} service he started a long {\color{orange} career} at the BBC.}             \\
\multicolumn{5}{l}{{\color{red} After} achieving his {\color{blue} diplomatic} post he initiated a later {\color{orange} time} at the university.}             \\
\multicolumn{5}{l}{{\color{red} After} failing his {\color{blue} military} initiation he found a meaningful {\color{orange} task} at the church.}             \\
\multicolumn{5}{l}{{\color{red} After} qualifying his {\color{blue} northern} bank he established a busy {\color{orange} series} at the site.}             \\
\multicolumn{5}{l}{{\color{red} After} abandoning his {\color{blue} postal} background he obtained a commercial {\color{orange} post} at the ministry.}             \\
\multicolumn{5}{l}{{\color{red} After} undergoing his {\color{blue} political} discharge he developed a second {\color{orange} attachment} at the secretariat.}             \\
\end{tabular}
}
\caption*{Figure 1:  A few structurally-equivalent sentences. The first sentence is original sentence from Wikipedia, and the sentences below it were generated by the process of repeated BERT substitution. Some sets of corresponding words--that is, words that share the same structural function--are highlighted in the same color.}

==> main.tex <==
% \documentclass[11pt,a4paper]{article}
% \usepackage[hyperref]{emnlp2020}
% % Optional math commands from https://github.com/goodfeli/dlbook_notation.
% \input{math_commands.tex}

% \usepackage{hyperref}
% \usepackage{url}
% \usepackage{float}


% % Own pacakges
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}

% \newcommand{\yanai}[1]{\textcolor{blue}{[YE: #1]}}
% \newcommand{\shauli}[2]{\textcolor{green}{[SR: #1]}}
% \newcommand{\yg}[3]{\textcolor{red}{[YG: #1]}}
% \newcommand{\T}{{\scriptscriptstyle \top}}

% \title{Unsupervised Distillation of Syntactic Information from Contextualized Word Representations}
% \date{August 2019}

% \begin{document}

% \maketitle

% \begin{abstract}
% \input{01_abstract}

% \end{abstract}


% \input{10_intro}

% \input{20_related}

% \input{30_method}

% \input{40_experiments}

% \input{50_conclusion}


% \bibliography{anthology,emnlp2020}
% \bibliographystyle{acl_natbib}

% \appendix

% \input{99_appendix}



% \end{document}


==> tables/closest_sentence_results.tex <==
\centering\begin{tabular}{lccc} \hline 
       & All sentences & Short sentences & Long sentences \\ \hline
Before & 0.011        & 0.030          & 0.00183        \\
After  & 0.017        & 0.045          & 0.00200        \\
Ratio  & 1.549         & 1.52           & 1.092 \\   \hline     
\end{tabular}
\caption{\label{tbl:closest_sentence_results} Results in the closest-sentence queries, before and after the application of the syntactic transformation.}
